An Embarrassingly Simple Way to Optimize Orthogonal Matrices at Scale

Orthogonality constraints are ubiquitous in robust and probabilistic machine learning. Unfortunately, current optimizers are computationally expensive and do not scale to problems with hundreds or thousands of constraints. One notable exception is the Landing algorithm (Ablin et al., 2024) which, however comes at the expense of temporarily relaxing orthogonality. In this work, we revisit and improve on the ideas behind Landing, enabling the inclusion of modern adaptive optimizers while ensuring that orthogonal constraints are effectively met. Remarkably, these improvements come at little to no cost, and reduce the number of required hyperparemeters. Our algorithm POGO is fast and GPU-friendly, consisting of only 5 matrix products, and in practice maintains orthogonality at all times. On several challenging benchmarks, POGO greatly outperforms recent optimizers and shows it can optimize problems with thousands of orthogonal matrices in minutes while alternatives would take hours. As such, POGO sets a milestone to finally exploit orthogonality constraints in ML at scale. A PyTorch implementation of POGO is publicly available at https://github.com/adrianjav/pogo.

==> math_commands.tex <==
\RequirePackage{mathtools}
\RequirePackage{amsmath,amsfonts,bm}
\RequirePackage{suffix}

\newcommand{\equationPunctuation}[1]{\,{#1}}
\let\eqp\equationPunctuation

\newcommand{\thetab}{{\boldsymbol{\theta}}}
\newcommand{\betab}{{\boldsymbol{\beta}}}
\newcommand{\pib}{{\boldsymbol{\pi}}}
\newcommand{\taub}{{\boldsymbol{\tau}}}
\newcommand{\psib}{{\boldsymbol{\psi}}}
\newcommand{\phib}{{\boldsymbol{\phi}}}
\newcommand{\omegab}{{\boldsymbol{\omega}}}
\newcommand{\etab}{{\boldsymbol{\eta}}}
\newcommand{\sigmab}{{\boldsymbol{\sigma}}}

\newcommand{\Thetab}{{\boldsymbol{\Theta}}}

\newcommand{\distribution}[1][]{\ensuremath{{P}_{#1}}\xspace}
\newcommand{\cumulative}[1][]{\ensuremath{F_{#1}}\xspace}
\newcommand{\empcumulative}[1][]{\ensuremath{\hat F_{#1}}\xspace}
\newcommand{\pushforward}[2]{{#1}_{\#} {#2}}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclarePairedDelimiter{\Ebrackets}{[}{]}
\newcommand{\Expect}[2][]{\E_{#1}\Ebrackets{#2}}
\WithSuffix\newcommand\Expect*[2][]{\E_{#1}\Ebrackets*{#2}}

\DeclareMathOperator{\V}{\mathbb{V}}
\newcommand{\Var}[2][]{\V_{#1}\Ebrackets{#2}}

\newcommand{\normal}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\uniform}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\categorical}{\ensuremath{\operatorname{Cat}}\xspace}
\newcommand{\bernoulli}{\ensuremath{\operatorname{Bern}}\xspace}
\newcommand{\binomial}{\ensuremath{\operatorname{Bin}}\xspace}
\newcommand{\lognormal}{\ensuremath{\operatorname{Log-normal}}\xspace}
\newcommand{\poisson}{\ensuremath{\operatorname{Poiss}}\xspace}
\newcommand{\exponentialdistribution}{\ensuremath{\operatorname{Exp}}\xspace}
\newcommand{\betadistribution}{\ensuremath{\operatorname{Beta}}\xspace}

\newcommand{\identity}{\ensuremath{\mI}}
\newcommand{\indicator}[1]{\ensuremath{\small [\,#1\,]}}
\newcommand{\ones}{\ensuremath{\mathbf{1}}\xspace}
\newcommand{\zeroes}{\ensuremath{\mathbf{0}}\xspace}
\DeclareMathOperator{\tr}{Trace}

\DeclareMathOperator*{\avg}{avg}
\DeclareMathOperator*{\med}{med}
\DeclareMathOperator*{\std}{std}

\let\cossim\cos


\usepackage{suffix}
\usepackage{xparse}
\usepackage{mathtools}

\def\rL{{\textnormal{L}}}
\def\rvL{{\mathbf{L}}}
\def\ervL{{\textnormal{L}}}

\def\rM{{\textnormal{M}}}
\def\rvM{{\mathbf{M}}}
\def\ervM{{\textnormal{M}}}

\def\rU{{\textnormal{U}}}
\def\rvU{{\mathbf{U}}}
\def\ervU{{\textnormal{U}}}

\DeclareMathOperator{\littleo}{\ensuremath{o}}
\DeclareMathOperator{\bigO}{\ensuremath{\mathcal{O}}}

\newcommand{\tensor}[1]{\ensuremath{\mathsf{#1}}}
\renewcommand{\vec}{\operatorname{vec}}
\newcommand{\D}{\mathrm{D}}
\newcommand{\Gmat}{\mathrm{G}}
\newcommand{\F}{\mathrm{F}}
\newcommand{\He}{\mathrm{H}}
\newcommand{\HeCal}{\mathcal{H}}
\newcommand*\dif{\mathop{}\!\mathrm{d}}
\newcommand{\average}[1]{\overline{ #1 }}

\newcommand{\Loss}{\mathcal{L}}
\newcommand{\jac}{\mathrm{J}}
\newcommand{\lin}[1]{\left\langle #1 \right\rangle}
\DeclareMathOperator{\trace}{Tr}

\newcommand{\nablasquaredsub}[1]{
  \nabla^{\kern -.0em \raise.1em\hbox{\tiny$2$}} {\kern -.6em \raise-.1em\hbox{\tiny$#1$}}{}
}
\newcommand{\nablasub}[1]{
  \nabla {\kern -.2em \raise-.1em\hbox{\tiny$#1$}}{}
}

\colorlet{captioncolor}{.}
\newcommand{\figleft}{{\color{captioncolor}(left)}\xspace}
\newcommand{\figcenter}{{\color{captioncolor}(center)}\xspace}
\newcommand{\figright}{{\color{captioncolor}(right)}\xspace}
\newcommand{\figtop}{{\color{captioncolor}(top)}\xspace}
\newcommand{\figbottom}{{\color{captioncolor}(bottom)}\xspace}
\newcommand{\Figleft}{{\color{captioncolor}(Left)}\xspace}
\newcommand{\Figcenter}{{\color{captioncolor}(Center)}\xspace}
\newcommand{\Figright}{{\color{captioncolor}(Right)}\xspace}
\newcommand{\Figtop}{{\color{captioncolor}(Top)}\xspace}
\newcommand{\Figbottom}{{\color{captioncolor}(Bottom)}\xspace}
\newcommand{\captiona}{{\color{captioncolor}(a)}\xspace}
\newcommand{\captionb}{{\color{captioncolor}(b)}\xspace}
\newcommand{\captionc}{{\color{captioncolor}(c)}\xspace}
\newcommand{\captiond}{{\color{captioncolor}(d)}\xspace}

\colorlet{itemcolor}{maincolor}
\newcommand{\itemi}{{\bfseries \color{itemcolor} i)}\xspace}
\newcommand{\itemii}{{\bfseries \color{itemcolor} ii)}\xspace}
\newcommand{\itemiii}{{\bfseries \color{itemcolor} iii)}\xspace}
\newcommand{\itemiv}{{\bfseries \color{itemcolor} iv)}\xspace}
\newcommand{\itemv}{{\bfseries \color{itemcolor} v)}\xspace}

\newcommand{\newterm}[1]{{\bf #1}}

\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvi{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\newcommand{\vecvar}[1]{\ensuremath{\bm{\mathrm{#1}}}}
\newcommand{\va}{\vecvar{a}}
\newcommand{\vb}{\vecvar{b}}
\newcommand{\vc}{\vecvar{c}}
\newcommand{\vd}{\vecvar{d}}
\newcommand{\ve}{\vecvar{e}}
\newcommand{\vell}{\vecvar{\ell}}
\newcommand{\vf}{\vecvar{f}}
\newcommand{\vg}{\vecvar{g}}
\newcommand{\vh}{\vecvar{h}}
\newcommand{\vi}{\vecvar{i}}
\newcommand{\vj}{\vecvar{j}}
\newcommand{\vk}{\vecvar{k}}
\newcommand{\vl}{\vecvar{l}}
\newcommand{\vm}{\vecvar{m}}
\newcommand{\vn}{\vecvar{n}}
\newcommand{\vo}{\vecvar{o}}
\newcommand{\vp}{\vecvar{p}}
\newcommand{\vq}{\vecvar{q}}
\newcommand{\vr}{\vecvar{r}}
\newcommand{\vs}{\vecvar{s}}
\newcommand{\vt}{\vecvar{t}}
\newcommand{\vu}{\vecvar{u}}
\newcommand{\vv}{\vecvar{v}}
\newcommand{\vw}{\vecvar{w}}
\newcommand{\vx}{\vecvar{x}}
\newcommand{\vy}{\vecvar{y}}
\newcommand{\vz}{\vecvar{z}}

\newcommand{\vA}{\vecvar{A}}
\newcommand{\vB}{\vecvar{B}}
\newcommand{\vC}{\vecvar{C}}
\newcommand{\vD}{\vecvar{D}}
\newcommand{\vE}{\vecvar{E}}
\newcommand{\vF}{\vecvar{F}}
\newcommand{\vG}{\vecvar{G}}
\newcommand{\vH}{\vecvar{H}}
\newcommand{\vI}{\vecvar{I}}
\newcommand{\vJ}{\vecvar{J}}
\newcommand{\vK}{\vecvar{K}}
\newcommand{\vL}{\vecvar{L}}
\newcommand{\vM}{\vecvar{M}}
\newcommand{\vN}{\vecvar{N}}
\newcommand{\vO}{\vecvar{O}}
\newcommand{\vP}{\vecvar{P}}
\newcommand{\vQ}{\vecvar{Q}}
\newcommand{\vR}{\vecvar{R}}
\newcommand{\vS}{\vecvar{S}}
\newcommand{\vT}{\vecvar{T}}
\newcommand{\vU}{\vecvar{U}}
\newcommand{\vV}{\vecvar{V}}
\newcommand{\vW}{\vecvar{W}}
\newcommand{\vX}{\vecvar{X}}
\newcommand{\vY}{\vecvar{Y}}
\newcommand{\vZ}{\vecvar{Z}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evyhat{{\hat{y}}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mGtilde{\bm{\tilde{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mWhat{{\bm{\hat{W}}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mPi{{\bm{\Pi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}
\def\mDelta{{\bm{\Delta}}}
\def\mStilde{\bm{\tilde{\mS}}}
\def\mGtilde{\bm{\tilde{\mG}}}
\def\mGoverline{{\bm{\overline{G}}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sYhat{{\hat{\mathbb{Y}}}}
\def\sZ{{\mathbb{Z}}}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\def\sOmega{{\mathbbold{\Omega}}}
\def\sPhi{{\mathbbold{\Phi}}}
\def\sTheta{{\mathbbold{\Theta}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}
\def\emPi{{\Pi}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\mathrm{data}}}
\newcommand{\ptrain}{\hat{p}_{\mathrm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\mathrm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\ifcsname laplace\endcsname%
    \renewcommand{\laplace}{\mathrm{Laplace}}%
\else%
    \newcommand{\laplace}{\mathrm{Laplace}}%
\fi


\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\onehot}{\mathrm{onehot}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}


\newcommand{\parents}[1]{{\ensuremath{\mathrm{pa}_{#1}}\xspace}}
\newcommand{\ancestors}[1]{{\ensuremath{\mathrm{an}_{#1}}\xspace}}
\newcommand{\children}[1]{{\ensuremath{\mathrm{ch}_{#1}}\xspace}}


\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\vmap}{vmap}
\DeclareMathOperator{\reshape}{reshape}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\eig}{eig}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\vecspan}{span}
\DeclareMathOperator{\overlap}{overlap}
\DeclareMathOperator{\Cat}{Cat}

\newcommand{\hess}[1]{\ensuremath{\mathrm{H}_{#1}}}

\newcommand{\Dtrain}{\ensuremath{\sD_{\mathrm{train}}}}
\newcommand{\Dtest}{\ensuremath{\sD_{\mathrm{test}}}}
\newcommand{\Dvalid}{\ensuremath{\sD_{\mathrm{valid}}}}


\DeclarePairedDelimiterX{\KLdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\KLdiv}{\KL\KLdivx}

\NewDocumentCommand{\giventhat}{O{\;|} m m}{#2#1\;#3}

\let\ab\allowbreak




==> paper_commands.tex <==
\let\figbf\textbf

\newcommand{\ours}{POGO\xspace}
\newcommand{\ourspl}{POGO\xspace}
\newcommand{\Ours}{\expandafter\MakeUppercase\ours}
\newcommand{\Ourspl}{\expandafter\MakeUppercase\ourspl}
\newcommand{\ourslong}{Proximal One-step Geometric Orthoptimizer\xspace}




\newcommand{\indexone}{i}%
\newcommand{\indextwo}{j}%
\NewDocumentCommand{\Stiefel}{O{\sR} m m O{}}{\ensuremath{\operatorname{St}^{#4}({#2},{#3})}\xspace}
\newcommand{\tangent}[1][\mX]{\ensuremath{\mathcal{T}_{#1}}\xspace}
\newcommand{\grad}[1][f(\mX)]{\ensuremath{\operatorname{grad}({#1})}\xspace}
\DeclareMathOperator{\dist}{\mathcal{N}}
\DeclarePairedDelimiterX\innerp[2]{\langle}{\rangle}{#1,#2}
\NewDocumentCommand{\innerfro}{m m}{\ensuremath{\Tr({#2^\top}\!{#1})}}

\newcommand{\methodname}[1]{\texttt{\small #1}}
\newcommand{\pogo}{\methodname{\ours}\xspace}
\newcommand{\rgd}{\methodname{RGD}\xspace}
\newcommand{\landing}{\methodname{Landing}\xspace}
\newcommand{\rsdm}{\methodname{RSDM}\xspace}
\newcommand{\landingpc}{\methodname{LandingPC}\xspace}
\newcommand{\slpg}{\methodname{SLPG}\xspace}


\DeclareMathOperator{\Skew}{Skew}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\BO}{BO}



==> tikz.tex <==

\RequirePackage{tikz,pgfplots}

\usetikzlibrary{
    shapes,
    pgfplots.groupplots,
    shadings,
    calc,
    arrows,
    backgrounds,
    colorbrewer,
    shadows.blur,
    external,
    shapes,
    shapes.arrows,
    shapes.symbols,
    arrows.meta,
    positioning, 
    decorations.pathreplacing,
    intersections,
    cd,
    babel, %
    fit %
}


\tikzstyle{varcurvestyle}=[
    smooth,
    thick,
    mark=none,
    domain=1:1000,
    samples=100,
]

\tikzstyle{ballstyle}=[
    smooth,
    thick,
    mark=none,
    samples=500,
]

